Dynamic Joint Uplink and Downlink Optimization for Uplink and Downlink Decoupling-Enabled 5G Heterogeneous Networks

The concept of user-centric and personalized service in the fifth generation (5G) mobile networks encourages technical solutions such as dynamic asymmetric uplink/downlink resource allocation and elastic association of cells to users with decoupled uplink and downlink (DeUD) access. In this paper we develop a joint uplink and downlink optimization algorithm for DeUD-enabled wireless networks for adaptive joint uplink and downlink bandwidth allocation and power control, under different link association policies. Based on a general model of inter-cell interference, we propose a three-step optimization algorithm to jointly optimize the uplink and downlink bandwidth allocation and power control, using the fixed point approach for nonlinear operators with or without monotonicity, to maximize the minimum level of quality of service satisfaction per link, subjected to a general class of resource (power and bandwidth) constraints. We present numerical results illustrating the theoretical findings for network simulator in a real-world setting, and show the advantage of our solution compared to the conventional proportional fairness resource allocation schemes in both the coupled uplink and downlink (CoUD) access and the novel link association schemes in DeUD.

==> appendices.tex <==

\appendix
\begin{proof} 

{\it Proposition \ref{prop:Duality}:}
For any fixed BS assignment $\hat{\ve{b}}$, denote $\hW:=\ma{W}_{\hat{\ve{b}}}$ and $\hV:=\Vb$ for convenience,  the optimal downlink power solution $\hat{\ve{q}}^{\dl}$ for problem \eqref{eqn:LB_dl} satisfies \cite{stanczak2009fundamentals}
		\begin{equation}
		\vspace{-0.2em}
		\ma{\Lambda}^{\dl} \hat{\ve{q}}^{\dl}=\frac{1}{C^{\dl}(\hat{\ve{b}},\Pm)} \hat{\ve{q}}^{\dl}, \hat{\ve{q}}^{\dl}\in\R_{+}^C
		\label{eqn:DL_matrixEqua}
		\vspace{-0.2em}
		\end{equation}
		where $\ma{\Lambda}^{\dl}\in\R_{+}^{C\times C}$ is defined as
		\begin{equation}
		\vspace{-0.2em}
		\ma{\Lambda}^{\dl}:=\ma{\Gamma}\ma{\Psi}\left[\ma{A}\hV^T\Aa^T+\frac{1}{\Pm}\ve{z}^{\dl}\ve{1}_C^T\right].
		\label{eqn:DL_Lambda}
		\vspace{-0.2em}
		\end{equation}
		we denote $\ma{\Gamma}:=\diag\{\gamma_1,\ldots, \gamma_C\}$, $C^{\dl}(\hat{\ve{b}},\Pm)=\max_{\ve{q}\geq 0}\min_c U_c^{(\text{d},1)}/\gamma_c$ subject to $\|\ve{q}\|_1\leq \Pm$, and 
		$\ve{1}_C$ is a C-dimensional all-one vector.
		\eqref{eqn:DL_matrixEqua} and \eqref{eqn:DL_Lambda} are derived by writing the utility fairness $U_c^{(\text{d},1)}/\gamma_c=C^{\dl}(\hat{\ve{b}}, \Pm)$ for all $c\in\set{C}$ and the power constraint $\|\ve{q}^{\dl}\|_1=\Pm$ with matrix notation. Targets $\ve{\gamma}$ is feasible if and only if $C^{\dl}(\hat{\ve{b}},\Pm)>1$. 
		
		Similarly, the optimal uplink power solution $\hat{\ve{q}}^{\ul}$ for uplink problem \eqref{eqn:LB_ul} needs to satisfy 
		\begin{equation}
		\vspace{-0.2em}
		\ma{\Lambda}^{\ul}\hat{\ve{q}}^{\ul}=\frac{1}{C^{\ul}(\hat{\ve{b}},\Pm)} \hat{\ve{q}}^{\ul}, \hat{\ve{q}}^{\ul}\in\R_{+}^C
		\label{eqn:UL_matrixEqua}
		\vspace{-0.2em}
		\end{equation}
		where $\ma{\Lambda}^{\ul}\in\R_{+}^{C\times C}$ is defined as
		\begin{equation}
		\vspace{-0.2em}
		\ma{\Lambda}^{\ul}:=\ma{\Gamma}\ma{\Psi}\left[\ma{A}\hW\Aa^T+\frac{1}{\Pm}\ve{z}^{\ul}\ve{1}_C^T\right].
		\label{eqn:UL_Lambda}
		\vspace{-0.2em}
		\end{equation}
		where $\ve{z}^{\ul}:=\ma{A}\ve{\sigma}^{\ul}$, i.e., $z_c^{\ul}=\Sigma_{\text{tot}}/C$ for all $c\in\set{C}$. 
		
		The balanced level $C^{\dl}(\hat{\ve{b}},\Pm)$ and
		$C^{\ul}(\hat{\ve{b}},\Pm)$ are the reciprocal spectral radius of the
		nonnegative extended coupling matrix $\ma{\Lambda}^{\dl}$ and
		$\ma{\Lambda}^{\ul}$. Moreover, according to Perron-Frobenius theorem, if both $\ma{\Lambda}^{\dl}$ and
		$\ma{\Lambda}^{\ul}$ are irreducible, they have unique real spectral radius and their corresponding eigenvectors (power allocation) have strictly positive components. By comparing the interference terms in
		\eqref{eqn:DL_Lambda} and \eqref{eqn:UL_Lambda}, we have
		$(\ma{A}\hV^T\Aa^T)^T=\Aa\hV\ma{A}^T=\ma{A}\diag\{\ve{\alpha}\}\hV
		\ma{I}\ma{A}^T=\ma{A}\diag\{\ve{\alpha}\}\hV\diag^{-1}\{\ve{\alpha}\}\diag\{\ve{\alpha}\}
		\ma{A}^T=\ma{A}\hW^T\Aa^T$. By comparing the noise terms we have
		$\ve{z}^{\ul}=\frac{1}{C} \ve{1}_C{\ve{z}^{\dl}}^T\ve{1}_C$ (by using
		$z_c^{\ul}=\Sigma_{\text{tot}}/C$ for all $c\in\set{C}$), thus
		$\ve{z}^{\ul}\ve{1}_C^T=\frac{1}{C}
		\ve{1}_C{\ve{z}^{\dl}}^T\ve{1}_C\ve{1}_C^T=\ve{1}_C{\ve{z}^{\dl}}^T=(\ve{z}^{\dl}\ve{1}_C^T)^T$. By
		using the properties of spectral radius $\rho(\ma{X})=\rho(\ma{X}^T)$
		and $\rho(\ma{X}\ma{Y})=\rho(\ma{Y}\ma{X})$ we have that
		$\rho(\ma{\Lambda}^{\dl})=\rho(\ma{\Lambda}^{\ul})$ and thus
		$C^{\dl}(\hat{\ve{b}},P^{\text{max}})=C^{\ul}(\hat{\ve{b}},P^{\text{max}})$. Notice
		that the network duality holds for any given BS assignment
		$\hat{\ve{b}}$, the achievable utility regions are the same for both
		the downlink problem \eqref{eqn:LB_dl} and uplink problem
		\eqref{eqn:LB_ul}.
		\end{proof}
